Emergency Incident Detection from Crowdsourced Waze Data using Bayesian Information Fusion

The number of emergencies have increased over the years with the growth in urbanization. This pattern has overwhelmed the emergency services with limited resources and demands the optimization of response processes. It is partly due to traditional `reactive' approach of emergency services to collect data about incidents, where a source initiates a call to the emergency number (e.g., 911 in U.S.), delaying and limiting the potentially optimal response. Crowdsourcing platforms such as Waze provides an opportunity to develop a rapid, `proactive' approach to collect data about incidents through crowd-generated observational reports. However, the reliability of reporting sources and spatio-temporal uncertainty of the reported incidents challenge the design of such a proactive approach. Thus, this paper presents a novel method for emergency incident detection using noisy crowdsourced Waze data. We propose a principled computational framework based on Bayesian theory to model the uncertainty in the reliability of crowd-generated reports and their integration across space and time to detect incidents. Extensive experiments using data collected from Waze and the official reported incidents in Nashville, Tenessee in the U.S. show our method can outperform strong baselines for both F1-score and AUC. The application of this work provides an extensible framework to incorporate different noisy data sources for proactive incident detection to improve and optimize emergency response operations in our communities.

==> archive/PreviousWriteup.tex <==
Crowdsourced data (such as Twitter) represents another important source of data for studying traffic crashes \cite{d2015real,gu2016twitter}. In their study,  Amin-Naseri et al \cite{amin2018evaluating} considered a temporal resolution of 20 minutes and a spatial resolution of 2.5 mile for matching the Waze data to an incident. In addition to spatio-temporal matching, they also considered semantic matching, where they matched road names, directions and accident types. They stated that Waze data covered 43.2\% of the official traffic incident database (ATMS). In their analysis, they obtained a 95\% confidence interval of [0.36, 0.39] miles and [0.8, 1.3] minutes for spatial and temporal resolution respectively considering those data that are common to Waze and ATMS.




\begin{itemize}
    \item We need to mention that we are using only reliability for aggregating waze reports (No report rating and confidence scores) -- mention that reliability is an aggregated score of the two features. We don't know how they are aggregated, and that score is directly available from a waze report
    \item Waze reports with the same UUID are assumed to be different waze reports by several wazers. They are not duplicates but multiple information sources from several wazers
\end{itemize}


In this paper, we consider four attributes from each waze report (w) for incident prediction: reliability ($r$), latitude ($l$), longitude ($g$) and time stamp ($t$)

As discussed in Section \ref{sec:dataset}, the reliability score is an integer value between 1 and 10. In order to calculate incident prediction, we need to aggregate multiple waze reports with different reliability scores. Since reliability scores are empirical scores, we do not have a mathematical framework to aggregate them.

We also know that as the reliability increases, the overall confidence regarding the report incident also increases. Therefore, we associated every possible reliability score with a probability value. If $r$ is the reliability score ($ r \in \mathbb{Z}, 1\leq r \leq 10$), then the associated probability measure is denoted as $p$ ($0\leq p \leq 1$). We will have ten different probability values corresponding to the ten reliability values. However, the associated probability values are unknown and need to be learnt from data. Moreover if $r_i$ and $r_j$ are two different reliability scores such that $r_i < r_j$, then the associated probability values $p_i$ and $p_j$ also follow that $p_i < p_j$.

In the learning state, our goal is to compare the information gained from multiple waze reports, and comparing it with a validated incident database. In the prediction phase, we use the trained model to calculate the probability of an incident happening in a given region. In both learning and prediction phases, the aggregation of multiple waze reports is an important analysis, which is disscussed below.

Let us consider fusion of multiple waze reports within a given cluster and in a time window ($T$). Assume that there are $n$ waze reports, denoted as $\mathbf{w_T} = w^i_T, i=1\dots n$. The latitude and longitude values are used in the clustering process, and the timestamp is used for temporal discretization.

Let $R_j, j=1\dots k$ represent the $k$ regions (road segments). Let $P(R_{j}|\mathbf{w_{T-1}})$ represent the incident probability after analyzing waze reports up to time step $T-1$. This probability becomes the prior probability for the next time interval $T$. Using $\mathbf{w_T}$, we update the incident probabilities in regions covered by them. The updated probabilities can be calculated using Bayes theorem as 

\begin{equation}
\label{eqn:Bayes}
\begin{aligned}
     P(R_{j}|\mathbf{w_T}) = & \dfrac{P(\mathbf{w_T}|R_j) \times P(R_{j})}{P(\mathbf{w_T})}\\
     & \propto P(\mathbf{w_T}|R_j) \times P(R_{j,T})  
\end{aligned}
\end{equation}

In Eq. \ref{eqn:Bayes}, $P(R_{j})$ and $P(R_{j}|\mathbf{w_T})$ represent the prior and posterior incident probabilities in region $R_j$ at time interval $T$. $P(\mathbf{w_T}|R_j)$ represents the likelihood of observing $\mathbf{w_T}$ given that an incident occurred in region $R_j$. Assuming all waze reports are independent to each other, we have

\begin{equation}
\label{eqn:ind}
    P(\mathbf{w_T}|R_j) = \prod_{i=1}^n P(w^i_T|R_j)
\end{equation}

In Eq. \ref{eqn:ind}, $P(w^i_T|R_j)$ represents the probability that the $i^{th}$ waze report at time interval $T$ represents an incident in region $R_j$. We calculate this probability in two steps. In the first step, we calculate the probability that a waze report corresponds to an incident. In the second step, we calculate the probability that the incident corresponds to region $R_j$.

Let $P(I^i_T=0)$ and $P(I^i_{T}=1)$ represent the probabilities that the $i^{th}$ waze report at time interval $T$ correspond to absence and presence of an incident respectively. Therefore,$P(I^i_T=0) + P(I^i_T=1) = 1$.

We know that a waze report is filed by a user (Wazer) based on his/her perception. Therefore, it is possible that the Wazer can be incorrect; this uncertainty is captured by the reliability measure: $r^i_T$. Therefore, the incident probability can be calculated as $P(I^i_{T}=1) = p^i_T$ and thus, $P(I^i_{T}=0) = 1-p^i_T$

% \begin{equation}
% \label{eqn:incident_prob}
% \begin{aligned}
%     P(I^i_{T}=1) = &P(I^i_{T}=1|C^i_T=0)P(C^i_T=0) + \\ &P(I^i_{T}=1|C^i_T=1)P(C^i_T=1)    
% \end{aligned}
% \end{equation}


% In Eq. \ref{eqn:incident_prob}, $P(I^i_{T}=1|C^i_T=0)$ and $P(I^i_{T}=1|C^i_T=1)$ is the incident probabilities when a wazer is reliable and  unreliable respectively. Hence, $P(I^i_{T}=1|C^i_T=0)$ is equal to the incident probability ($i^i_T$) available in the waze report. When the wazer is unreliable, we assume an equal probability of an incident happening, i.e., $P(I^i_{T}=1|C^i_T=1) = 0.5$. Therefore, Eq. \ref{eqn:incident_prob} can be calculated as 

% \begin{equation}
%     P(I^i_{T}=1) = i^i_T\times u^i_T + 0.5 \times (1-u^i_T) 
% \end{equation}

After calculating the incident probability associated with a waze report $w^i_T$, we now calculate the likelihood that the incident occurred in region $R_j$. Every waze report comes with a location information (latitude/longitude values). 

Usually, after a user identifies an incident, it will take some time for the user to report the incident. First, the user needs to process the incident, decide whether to file a waze report, and then file a waze report. The time it takes to perform the above three steps can vary between people; therefore, the location information does not correspond to the location of the incident, and the incident region is in ``close" vicinity to the location report in a waze report. This is incorporated by considering an uncertainty value $\delta$ in the reported latitude and longitude values. If $l_T^i$ and $g_T^i$ are the latitude and longitude values corresponding to $w_T^i$, then we consider an area covered between $l_T^i-\delta$ and $l_T^i+\delta$ along the latitude, and $g_T^i-\delta$ and $g_T^i+\delta$ along the longitude.

The likelihood $P(w^i_T|R_j)$ can be calculated as the product of the overlap between the area covered by the waze report and region $R_j$, and the incident probability. If $A(w_T^i)$ represents the area covered by $w_T^i$, and $\Omega(m,n)$ represents the overlap between two regions $m$ and $n$, them the likelihood can be calculated as 

\begin{equation}
\label{eqn:like_one}
    P(w^i_T|R_j) = P(I^i_{T}=1)\dfrac{\Omega(A(w^i_T), R_j)}{A(w^i_T)}
\end{equation}

Using Eqs. \ref{eqn:ind} and \ref{eqn:like_one}, we can calculate the overall likelihood considering all the $n$ waze reports as 

\begin{equation}
\label{eqn:overall_like}
    P(\mathbf{w_T}|R_j) = \prod_{i=1}^n P(I^i_{T}=1)\dfrac{\Omega(A(w^i_T), R_j)}{A(w^i_T)}
\end{equation}

Given the overall likelihood, the posterior incident probability in each region can be calculated using Eq. \ref{eqn:Bayes}. With time, the incident probabilities in various regions also changes. Here, let us introduce another parameter $\delta$, which corresponds to the minimum incident probability that should be reached within a region before notifying emergency response authorities. If $P(R_{j}|\mathbf{w_T}) \geq \delta$, we assume we have sufficient confidence that an incident occurred in region $R_j$ and notify the authorities.

The parameters that need to be estimated in the learning phase are (1) the probability values associated with the reliability values; (2) Threshold probability ($\delta$); and (3) Spatial and temporal resolution.

%When calculating the incident probability, we combine the waze reports from the previous time step ($T-1$) that are unused and the waze reports from the current time step ($T$). Let us denote the unused waze reports from $T-1$ as $\mathbf{w_{T-1}^u}$. The total available waze reports to be analyzed in the current time step are $\mathbf{w_{T-1}^u} \cup \mathbf{w_T}$. 




\section{Results and Discussion}
\label{sec:results}




\section{Conclusion}
\label{sec:conclude}




\begin{figure*}
    \centering
    \includegraphics[scale=0.7]{Picture1.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{AccidentReporting.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure*}

\textcolor{red}{New writeup}

Assume that it takes $t$ seconds to file a waze report after noticing an incident. The value of $t$ is not constant, and is assumed to follow a probability distribution $f(t)$, i.e., $\int_{t=0}^{\infty} f(t) dt = 1$. Let $x_n = (l_n, g_n), x_r = (l_r, g_r)$ represent the locations when the accident in noticed by a wazer and when the incident is reported.  Let $x_a = (l_a, g_a)$ represent the coordinates of the accident. Let $N(x_a)$ represent the area from which the accident can be noticed; this area can span multiple regions (green region in Figure XX, $x_n \in N(x_a)$. Let $R(x_a)$ represent the region from which an incident at $x_a$ will be reported (gray region in Figure XX,  $x_r \in R(x_a)$). In Figure XX, the gray area spans five regions: R1, R2, R3, R4, R6. All the reports coming from outside this region are considered irrelevant to the incident at $x_a$.


\begin{equation}
\begin{aligned}
     P(R_j, I=1|w_T) &= \dfrac{P(w_T, R_j, I=1)}{P(w_T)}\\
     &=\dfrac{\prod_{i=1}^n P(w_T^i, R_j, I=1)}{P(w_T)}\\
    %  &= \dfrac{P(w_T|R_j, I=1)P(R_j, I=1)}{P(w_T)}
\end{aligned}
\end{equation}

Here, $P(R_j, I=1)$ and $P(R_j, I=1|w_T)$ are the prior and posterior probabilities of an incident happening in region $R_j$. $P(w_T)$ is the probability of observing the waze reports $w_T$.

\begin{equation}
\begin{aligned}
&P(w_T) = P(w_T, I=1) + P(w_T, I=0)\\
&= \sum_{i=1}^k P(w_T, I=1, R_i) + P(w_T, I=0)\\
% &= \sum_{i=1}^k P(w_T|I=1, R_i) P(I=1, R_i) \\
% & \hspace{10mm}+ P(w_T|I=0)P(I=0) \\
% &= \sum_{j=1}^k \bigg(\prod_{i=1}^n P(w_T^i|I=1, R_j)\bigg) P(I=1, R_j) \\
% & \hspace{10mm}+ \bigg(\prod_{i=1}^n P(w_T^i|I=0)\bigg)P(I=0) \\
\end{aligned}
\end{equation}

Let $x_T^i = (l_T^i, g_T^i)$ denote the location of the waze report $w_T^i$.

\begin{equation}
\label{eqn:prob}
\begin{aligned}
& P(w_T^i, R_j, I=1) = p_T^i \int_{x_a\in R_j} P(x_T^i, x_a, I=1) dx_a\\
& = p_T^i\int_{x_a\in R_j} P(x_T^i|x=x_a, I=1) P(I=1, x_a)dx_a\\
%& = p_T^i \int_{x_a\in R_j} \bigg(\int_{x_n\in N(x_a)}P(x_T^i, x_n| I=1, x_a) dx_n \bigg)\\
%& \hspace{20mm} P(I=1, x_a)dx_a\\
%& = p_T^i\int_{x_a\in R_j} \bigg(\int_{x_n\in N(x_a)}P(x_T^i| x_n, I=1, x_a)\\
%& \hspace{20mm} P(x_n|I=1, x_a) dx_n \bigg) P(I=1, x_a)dx_a
\end{aligned}
\end{equation}


In Eq. \ref{eqn:prob}, $P(I=1, x_a)$ is the probability of an incident occurring at $x_a$ in region $R_j$. If $P(I=1, R_j)$ represents the probability of an incident happening in $R_j$, then $P(I=1, x_a) = \dfrac{P(I=1, R_j)}{A(R_j)}$ assuming a uniform probability of an incident all over region $R_j$, $A(.)$ is the area operator that computes the road area in a given region, and $A(R_j)$ is the total road area in $R_j$. $P(x_n|I=1, x_a)$ represents the probability that an incident at $x_a$ is noticed at location $x_n$ by a Wazer. Assuming a uniform distribution over the accident visibility region, $N(x_a)$, $P(x_n|I=1, x_a) = \dfrac{1}{A(N(x_a))}$, where $A(N(x_a))$ is the road area covered by region $N(x_a)$. $P(x_T^i| x_n, I=1, x_a)$ is the probability of observing a waze report $w_T^i$ with location $x_T^i$ due to an incident at $x_a$ and when the incident is noticed at $x_s$. Assuming a uniform velocity $v_t$ in the time period when an incident is noticed and when the incident is reported, the time lag can be calculated as $t^i_T = \dfrac{d(x_s, x_T^i)}{v_t}$, and with the available time lag distribution $f(t)$, the probability of $t^i_T$ can be calculated as $f(t=t^i_T)$. $p_T^i$ is the probability associated with the reliability $r_T^i$ of a waze report $w_T^i$.



\section{Outline}

Page 1.5: Introduction /Related Work \\
Page 2.25: Background \\
Page 3: Proposed Methodology \\
End of Page 5: More Proposed Methodology (Definitions, Assumptions, Dataset description, Proposed methods) \\
Page 6: Experimentation \\
Page 7: Results and Discussion \\
Page 8: Conclusion/Acknowledgement/References \\


\section{Analysis Example}

Consider the case in Figure 1 with four regions $R_1, R_2, R_3, R_4$. Assume that we have two waze reports in the first time step.

Let $I=1$ represent the event of an accident happening. $I=0$ represent no accident. If an accident occurs, it should occur in one of the four regions.

From historical data, we can obtain the prior accident probabilities in all the four regions. Lets call them $0.01,0.02, 0.03, 0.04$, i.e., $P(I=1, R_1) = 0.01$

Let $w_11, w_12$ represent the two waze reports in the first time step, and $p_{11} = 0.8, p_{12}=0.9$ be the probabilities (associated with their reliabilities)

\begin{equation}
    P(I=1, R_1|w_1, w_2) =   \dfrac{P(w_1, w_2|I=1, R_1) P(I=1, R_1)}{P(w_1, w_2)}
\end{equation}


Let us assume the overlap probabilities of $w_1$ with the four regions be 0.3, 0.2, 0.1 and 0.4.

Overlap with $w_2$ is 0.25, 0.15, 0.45,0.15. Let us compute the likelihood below.



    $P(w_1, w_2|I=1, R_1) = p_{11} 0.3 p_{12} 0.25 = 0.8 \times 0.3 \times 0.9 \times 0.25 = 0.054$


Therefore, likelihood times prior = $ 0.054 \times 0.01 = 0.00054$

Similarly, we will calculate likelihood times prior for R2, R3, and R4. For example, let their values be 0.00024, 0.00056, 0.00087 (these are random values).

So far, we calculated $P(I=1, R_1|w_1, w_2)$ which is the probability of an accident happening. One obvious question is - What is the probability that an accident did not happen at all, and the waze reports are all errors? This is calculated as 

$P(I=0|w_1, w_2) = \dfrac{P(w_1, w_2|I=0)P(I=0)}{P(w_1, w_2}$

$P(I=0)$ is the prior probability of an accident not happening at all. This is nothing but 1 - prior probabiltiies of accidents happening in various regions = 1 - 0.01 -0.02 - 0.03 - 0.04 = 0.9


$P(w_1, w_2|I=0)$ is the likelihood of observing the waze reports when an accident did not happen = $(1-p_{11})\times (1-p_{12}) = 0.1\times 0.2 = 0.02$

Likelihood times prior = 0.02 \times 0.9 = 0.018


Now we have likelihood times prior for all five cases (four cases with accident happening in four regions and one case without an accident)


We know that the posterior is proportional to likelihood times prior. Therefore, we can normalize all the above values.

\begin{equation}
    P(I=1, R_1|w_1, w_2) = \dfrac{0.00054}{0.00054 + 0.00024 + 0.00056 + 0.00087 + 0.018} = 0.02021
\end{equation}

The accident probabbility increased from 0.01 (prior) to 0.02021.
Similarly, we can calculate the other posterior probabilities as well. These will become the priors in the next time step






